A crowdsourcing approach to video quality assessment

The gold standard for measuring video quality is the subjective test, and the most prevalent is the ITU-T Rec. P.910, a lab-based subjective standard in use for the past two decades. However, in practice using ITU-T Rec. P.910 is slow, expensive, and requires a lab, which all create barriers to usage. As a result, most research papers that need to measure video quality don't use ITU-T Rec. P.910 but rather metrics that are not well correlated to subjective opinion. We provide an open-source extension of ITU-T Rec. P.910 based on crowdsourcing principles which address the speed, usage cost, and barrier to usage issues. We implement Absolute Category Rating (ACR), ACR with hidden reference (ACR-HR), Degradation Category Rating (DCR), and Comparison Category Rating (CCR). It includes rater, environment, hardware, and network qualifications, as well as gold and trapping questions to ensure quality. We have validated that the implementation is both accurate and highly reproducible compared to existing ITU-T Rec. P.910 lab studies.

==> junk.tex <==

%on focuses on subjective assessment of the audiovisual quality of Internet video and distribution quality in which the content transmitted over an unreliable link to a variety of (mobile) devices located in distracting environment. Compare to other standards, it includes multiple display technologies and testing environments (e.g. simulated office or public environment), provides flexibility on modifying the subjective scale, and considers applications with interaction effect that confound the data (e.g. impact of mobility on quality rating).

%Our pre-studies also showed that when participants are forced to perform this calibration task, their accuracy of recognizing number of shapes on follow up question increased by 20\%.


\begin{IEEEbiographynophoto}{Babak Naderi} 
received his Ph.D. degree for his work on crowdsourcing in 2017 and his Master of Science degree in 2012 both from the Technical University of Berlin. He was a senior research scientist at the Quality and Usability Lab, Technical University of Berlin until July 2022. He is currently a Senior Applied Scientist at Microsoft. His research interest includes Media Quality Assessment, the application of Deep Learning in Quality of Experience, Machine Learning, and Enhanced Crowdsourcing.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Ross Cutler} is a Partner Applied Scientist Manager at Microsoft where he leads the IC3-AI team to improve Teams/Skype audio/video quality and reliability and enable new functionality with AI. He has been with Microsoft since 2000, joining as a Researcher in Microsoft Research. He has published over 65 academic papers and has over 100 granted patents in the areas of computer vision, speech enhancement, machine learning, optics, and acoustics. Ross received his Ph.D. in Computer Science in 2000 in the area of computer vision from the University of Maryland, College Park.
\end{IEEEbiographynophoto}
